No Stripped Hydrogen in the Nebular Spectra of Nearby Type Ia Supernova 2011fe

A generic prediction of the single-degenerate model for Type Ia supernovae (SNe Ia) is that a significant amount of material will be stripped from the donor star (~0.5 Msun for a giant donor and ~0.15 Msun for a main sequence donor) by the supernova ejecta. This material, excited by gamma-rays from radioactive decay, would then produce relatively narrow (1000 km s-1) emission features observable once the supernova enters the nebular phase. Such emission has never been detected, which already provides strong constraints on Type Ia progenitor models. In this Letter we report the deepest limit yet on the presence of H-alpha emission originating from the stripped hydrogen in the nebular spectrum of a Type Ia supernova obtained using a high signal-to-noise spectrum of the nearby normal SN Ia 2011fe 274 days after B-band maximum light with the Large Binocular Telescope's Multi-Object Double Spectrograph. We put a conservative upper limit on the H-alpha flux of 3.14 x 10^-17 erg s-1 cm-2, which corresponds to a luminosity of 1.57 x 10^35 erg s-1. By scaling models from the literature, our flux limit translates into an upper limit of 0.001 Msun of stripped material. This is an order of magnitude stronger than previous limits. SN 2011fe was a typical Type Ia supernova, special only in its proximity, and we argue that lack of hydrogen emission in its nebular spectrum adds yet another strong constraint on the single degenerate class of models for SNe Ia.

==> tab1.tex <==
%\documentclass[preprint]{aastex}
%\pagestyle{empty}
%\begin{document}
%Table of Spectra.
\begin{deluxetable}{lrrrcrccccc}
%\tabletypesize{\scriptsize}
\tabletypesize{\tiny}
%\rotate{}
%\tablenum{1}
\tablewidth{450pt}
\tablecaption{Observations}
\tablehead{\colhead{} & 
\colhead{} &
\colhead{HJD} &
\colhead{P.A.} &
\colhead{Par. P.A.} &
\colhead{} & 
\colhead{Flux } &
\colhead{Seeing} &
\colhead{Exposure} &
\colhead{$r^{\prime}$} &
\colhead{Scale} \\
\colhead{UT Date} &
\colhead{Day} &
\colhead{$-$2,400,000} &
\colhead{(deg)} &
\colhead{(deg)} &
\colhead{Airmass} &
\colhead{standards} &
\colhead{(arcsec)} &
\colhead{(s)}  &
\colhead{(mag)}  &
\colhead{factor}  }
\startdata

2011 Nov 23.52 & 73.02  & 55889.02  &  $-78.0$ & $-84.3$ -- $-85.7$ & 1.60 -- 1.64 & Feige110, G191-B2B  & 0.8 / 0.9 &  360.0 / 360.0 & \nodata\tablenotemark{a} & 1.07\\

2012 Jan 2.54 & 113.05 & 55929.05 & $-124.4$ & $-134$ -- $-139$ & 1.11 -- 1.12 & Feige34 & 0.8 / 0.9 & 900.0 / 900.0 & $14.26 \pm 0.03$& 1.93 \\

2012 Mar 24.47 & 194.97 & 56010.97  & $-68.5$ & $110$ -- $124$ & 1.15 -- 1.24 & Feige67 & 0.5 / 0.7 & 2880.0 / 2160.0 & $16.35 \pm 0.01$ & 1.77 \\

2012 Apr 27.27 & 228.77 & 56044.77 & $-2.0$ & $-159$ -- $177$ & 1.07 -- 1.08 & HZ44, BD+33d2642  & 0.9 / 1.1 & 3600.0 / 3600.1 & $17.06 \pm 0.01$ & 2.20 \\

2012 Jun 12.16 & 274.66 & 56090.66 & $-32.7$ & $-177$ -- $129$ & 1.07 -- 1.13 & HZ44 & 0.7 / 0.7 & 7200.0 / 7200.0 & $17.95 \pm 0.01$ & 1.26 \\


\enddata \tablecomments{Observational and derived properties of our time series spectra of SN 2011fe. Days since maximum $B$ brightness assume JD $t_{B {\rm max}} = 2455816.0 \pm 0.3$ \citep{richmond12}. P.A. is the position angle of the spectrograph slit.  Par. P.A. and airmass give the range of parallactic angles and airmasses at the start of each separate observation, respectively. Standard stars were observed on the same night as science observations and, when multiple standards were available, the computed response functions from each standard were averaged. Seeing gives the FWHM for the red / blue channels of the spatial profile in the combined 2d spectra. Exposure times are given for the red / blue channels separately. $r^{\prime}$ magnitude is derived from the acquisition images. Each flux calibrated spectra was multiplied by a scale factor derived in the $R$- or $r^{\prime}$-band to place it on an absolute flux scale.}

\tablenotetext{a}{SN 2011fe was saturated in this epoch's acquisition images, so no reliable photometry was obtained.}

\label{tab:1}

\end{deluxetable}
% \clearpage
%\end{document}



==> values.tex <==
\newcommand{\WThreeeSigma}{\ensuremath{ 0.067} \AA}
\newcommand{\WMattila}{\ensuremath{ 5.8} \AA}
\newcommand{\WPlotted}{\ensuremath{ 0.12} \AA}
\newcommand{\WModel}{\ensuremath{ 0.081} \AA}
\newcommand{\MassLimitPlotted}{\ensuremath{ 0.001} \msun}
\newcommand{\MassLimit}{\ensuremath{ 5.8 \times 10^{-4}} \msun}
\newcommand{\MassLimitModel}{\ensuremath{ 7.0 \times 10^{-4}} \msun}
\newcommand{\Binning}{\ensuremath{ 4.0} \AA}
\newcommand{\SmoothWidth}{\ensuremath{           60} \AA}
\newcommand{\OneSigma}{\ensuremath{ 0.0024} \AA}
\newcommand{\PeakFluxMattila}{\ensuremath{ 6.71 \times 10^{-17}} erg s\ensuremath{^{-1}} cm\ensuremath{^{-2}} \AA\ensuremath{^{-1}}}
\newcommand{\PeakFluxLimit}{\ensuremath{ 7.79 \times 10^{-19}} erg s\ensuremath{^{-1}} cm\ensuremath{^{-2}} \AA\ensuremath{^{-1}}}
\newcommand{\PeakFluxLimitPlotted}{\ensuremath{ 1.34 \times 10^{-18}} erg s\ensuremath{^{-1}} cm\ensuremath{^{-2}} \AA\ensuremath{^{-1}}}
\newcommand{\PeakFluxLimitModel}{\ensuremath{ 9.40 \times 10^{-19}} erg s\ensuremath{^{-1}} cm\ensuremath{^{-2}} \AA\ensuremath{^{-1}}}
\newcommand{\FluxLimit}{\ensuremath{ 1.82 \times 10^{-17}} erg s\ensuremath{^{-1}} cm\ensuremath{^{-2}}}
\newcommand{\FluxLimitPlotted}{\ensuremath{ 3.14 \times 10^{-17}} erg s\ensuremath{^{-1}} cm\ensuremath{^{-2}}}
\newcommand{\FluxLimitModel}{\ensuremath{ 2.20 \times 10^{-17}} erg s\ensuremath{^{-1}} cm\ensuremath{^{-2}}}
\newcommand{\PeakFluxLimitSN}{\ensuremath{ 3.90 \times 10^{33}} erg s\ensuremath{^{-1}} \AA\ensuremath{^{-1}}}
\newcommand{\PeakFluxLimitSNPlotted}{\ensuremath{ 6.72 \times 10^{33}} erg s\ensuremath{^{-1}} \AA\ensuremath{^{-1}}}
\newcommand{\PeakFluxLimitSNModel}{\ensuremath{ 4.70 \times 10^{33}} erg s\ensuremath{^{-1}} \AA\ensuremath{^{-1}}}
\newcommand{\FluxLimitSN}{\ensuremath{ 9.13 \times 10^{34}} erg s\ensuremath{^{-1}}}
\newcommand{\FluxLimitSNPlotted}{\ensuremath{ 1.57 \times 10^{35}} erg s\ensuremath{^{-1}}}
\newcommand{\FluxLimitSNModel}{\ensuremath{ 1.10 \times 10^{35}} erg s\ensuremath{^{-1}}}
\newcommand{\BinsPerRes}{\ensuremath{ 1.13}}
\newcommand{\Angle}{\ensuremath{ 30.0}}

